An Error Bound for the Time-Sliced Thawed Gaussian Propagation Method

We study the time-sliced thawed Gaussian propagation method, which was recently proposed for solving the time-dependent Schr\"odinger equation. We introduce a triplet of quadrature-based analysis, synthesis and re-initialization operators to give a rigorous mathematical formulation of the method. Further, we derive combined error bounds for the discretization of the wave packet transform and the time-propagation of the thawed Gaussian basis functions. Numerical experiments in 1D illustrate the theoretical results.

==> 1-main latex/bibliography.tex <==
\begin{thebibliography}{MMC90}

\bibitem[BG20]{Blanes:2020}
S.~Blanes and V.~Gradinaru.
\newblock {High order efficient splittings for the semiclassical time-dependent
  Schr{\"o}dinger equation}.
\newblock {\em Journal of Computational Physics}, 405:109157, 2020.

\bibitem[BL20]{Bergold:2020u}
P.~Bergold and C.~Lasser.
\newblock {The Gaussian Wave Packet Transform via Quadrature Rules}.
\newblock Preprint on arXiv, {https://arxiv.org/abs/2010.03478}, 2020.

\bibitem[CDS03]{Chiani:2003}
M.~Chiani, D.~Dardari, and M.~K. Simon.
\newblock New exponential bounds and approximations for the computation of
  error probability in fading channels.
\newblock {\em IEEE Transactions on Wireless Communications}, 2(4):840--845,
  2003.

\bibitem[CK90]{Coalson:1990}
R.~D. Coalson and M.~Karplus.
\newblock {Multidimensional variational Gaussian wave packet dynamics with
  application to photodissociation spectroscopy}.
\newblock {\em The Journal of Chemical Physics}, 93(6):3919--3930, 1990.

\bibitem[CR12]{Combescure:2012}
M.~Combescure and D.~Robert.
\newblock {\em {Coherent States and Applications in Mathematical Physics}}.
\newblock Theoretical and Mathematical Physics. Springer Cham, {Second}
  edition, 2012.

\bibitem[DR07]{Davis:2007}
P.~J. Davis and P.~Rabinowitz.
\newblock {\em {Methods of Numerical Integration}}.
\newblock Academic Press, {Second} edition, 2007.

\bibitem[DT10]{Descombes:2010}
S.~Descombes and M.~Thalhammer.
\newblock {An exact local error representation of exponential operator
  splitting methods for evolutionary problems and applications to linear
  Schr{\"o}dinger equations in the semi-classical regime}.
\newblock {\em BIT Numerical Mathematics}, 50:729--749, 2010.

\bibitem[FF15]{Fornberg:2015}
B.~Fornberg and N.~Flyer.
\newblock {Solving PDEs with radial basis functions}.
\newblock {\em Acta Numerica}, 24:215--258, 2015.

\bibitem[FGL09]{Faou:2009}
E.~Faou, V.~Gradinaru, and C.~Lubich.
\newblock {Computing Semiclassical Quantum Dynamics with Hagedorn Wavepackets}.
\newblock {\em SIAM Journal on Scientific Computing}, 31(4):3027--3041, 2009.

\bibitem[FL06]{Faou:2006}
E.~Faou and C.~Lubich.
\newblock {A Poisson Integrator for Gaussian Wavepacket Dynamics}.
\newblock {\em Computing and Visualization in Science}, 9(2):45--55, 2006.

\bibitem[FLF11]{Fornberg:2011}
B.~Fornberg, E.~Larsson, and N.~Flyer.
\newblock {Stable Computations with Gaussian Radial Basis Functions}.
\newblock {\em SIAM Journal on Scientific Computing}, 33(2):869--892, 2011.

\bibitem[Fol89]{Folland:1989}
G.~B. Folland.
\newblock {\em {Harmonic Analysis in Phase Space}}.
\newblock Annals of Mathematics Studies. Princeton University Press, 1989.

\bibitem[FS98]{Feichtinger:1998}
H.~G. Feichtinger and T.~Strohmer.
\newblock {\em {Gabor Analysis and Algorithms: Theory and Applications}}.
\newblock Applied and Numerical Harmonic Analysis. Springer Science \& Business
  Media, 1998.

\bibitem[GG98]{Gerstner:1998}
T.~Gerstner and M.~Griebel.
\newblock {Numerical integration using sparse grids}.
\newblock {\em Numerical Algorithms}, 18(3):209--232, 1998.

\bibitem[GH14]{Gradinaru:2014}
V.~Gradinaru and G.~A. Hagedorn.
\newblock {Convergence of a semiclassical wavepacket based time-splitting for
  the Schr{\"o}dinger equation}.
\newblock {\em Numerische Mathematik}, 126(1):53--73, 2014.

\bibitem[Gr{\"o}01]{Grochenig:2001}
K.~Gr{\"o}chenig.
\newblock {\em {Foundations of Time-Frequency Analysis}}.
\newblock Applied and Numerical Harmonic Analysis. Springer Science \& Business
  Media, 2001.

\bibitem[Hag80]{Hagedorn:1980}
G.~A. Hagedorn.
\newblock {Semiclassical quantum mechanics. I. The {$\hbar \rightarrow 0$}
  limit for coherent states}.
\newblock {\em Communications in Mathematical Physics}, 71(1):77--93, 1980.

\bibitem[Hag98]{Hagedorn:1998}
G.~A. Hagedorn.
\newblock {Raising and Lowering Operators for Semiclassical Wave Packets}.
\newblock {\em Annals of Physics}, 269(1):77--104, 1998.

\bibitem[Hel75]{Heller:1975}
E.~J. Heller.
\newblock {Time‐dependent approach to semiclassical dynamics}.
\newblock {\em The Journal of Chemical Physics}, 62(4):1544--1555, 1975.

\bibitem[Hel76]{Heller:1976}
E.~J. Heller.
\newblock {Time dependent variational approach to semiclassical dynamics}.
\newblock {\em The Journal of Chemical Physics}, 64(1):63--73, 1976.

\bibitem[Hel81]{Heller:1981}
E.~J. Heller.
\newblock {Frozen Gaussians: A very simple semiclassical approximation}.
\newblock {\em The Journal of Chemical Physics}, 75(6):2923--2931, 1981.

\bibitem[Hig02]{Higham:2002}
N.~J. Higham.
\newblock {\em {Accuracy and Stability of Numerical Algorithms}}.
\newblock Other Titles in Applied Mathematics. Society for Industrial and
  Applied Mathematics (SIAM), {Second} edition, 2002.

\bibitem[HK84]{Herman:1984}
M.~F. Herman and E.~Kluk.
\newblock {A semiclasical justification for the use of non-spreading
  wavepackets in dynamics calculations}.
\newblock {\em Chemical Physics}, 91(1):27--34, 1984.

\bibitem[HLW06]{Hairer:2006}
E.~Hairer, C.~Lubich, and G.~Wanner.
\newblock {\em {Geometric Numerical Integration: Structure-Preserving
  Algorithms for Ordinary Differential Equations}}.
\newblock Springer Series in Computational Mathematics. Springer Berlin,
  Heidelberg, {Second} edition, 2006.

\bibitem[KLY19]{Kormann:2019}
K.~Kormann, C.~Lasser, and A.~Yurova.
\newblock {Stable Interpolation with Isotropic and Anisotropic Gaussians Using
  Hermite Generating Function}.
\newblock {\em SIAM Journal on Scientific Computing}, 41(6):A3839--A3859, 2019.

\bibitem[KMB16]{Kong:2016}
X.~Kong, A.~Markmann, and V.~S. Batista.
\newblock {Time-Sliced Thawed Gaussian Propagation Method for Simulations of
  Quantum Dynamics}.
\newblock {\em The Journal of Physical Chemistry A}, 120(19):3260--3269, 2016.

\bibitem[LL20]{Lasser:2020}
C.~Lasser and C.~Lubich.
\newblock {Computing quantum dynamics in the semiclassical regime}.
\newblock {\em Acta Numerica}, 29:229--401, 2020.

\bibitem[LQ09]{Leung:2009}
S.~Leung and J.~Qian.
\newblock {Eulerian Gaussian beams for Schr{\"o}dinger equations in the
  semi-classical regime}.
\newblock {\em Communications in Computational Physics}, 228(8):2951--2977,
  2009.

\bibitem[LRT13]{Liu:2013}
H.~Liu, O.~Runborg, and N.~M. Tanushev.
\newblock {Error Estimates for Gaussian Beam Superpositions}.
\newblock {\em Mathematics of Computation}, 82(282):919--952, 2013.

\bibitem[LS17]{Lasser:2017}
C.~Lasser and D.~Sattlegger.
\newblock {Discretising the Herman--Kluk Propagator}.
\newblock {\em Numerische Mathematik}, 137(1):119--157, 2017.

\bibitem[Lub08]{Lubich:2008}
C.~Lubich.
\newblock {\em {From Quantum to Classical Molecular Dynamics: Reduced Models
  and Numerical Analysis}}.
\newblock Zurich Lectures in Advanced Mathematics. European Mathematical
  Society (EMS), 2008.

\bibitem[Mar02]{Martinez:2002}
A.~Martinez.
\newblock {\em {An Introduction to Semiclassical and Microlocal Analysis}}.
\newblock Universitext. Springer New York, 2002.

\bibitem[MMC90]{Meyer:1990}
H.-D. Meyer, U.~Manthe, and L.S. Cederbaum.
\newblock {The multi-configurational time-dependent Hartree approach}.
\newblock {\em Chemical Physics Letters}, 165(1):73--78, 1990.

\bibitem[MQ02]{McLachlan:2002}
R.~I. McLachlan and G.~R.~W. Quispel.
\newblock {Splitting methods}.
\newblock {\em Acta Numerica}, 11:341--434, 2002.

\bibitem[Ose11]{Oseledets:2011}
I.~V. Oseledets.
\newblock {Tensor-Train Decomposition}.
\newblock {\em SIAM Journal on Scientific Computing}, 33(5):2295--2317, 2011.

\bibitem[OT09]{Oseledets:2009}
I.~V. Oseledets and E.~E. Tyrtyshnikov.
\newblock {Breaking the Curse of Dimensionality, Or How to Use SVD in Many
  Dimensions}.
\newblock {\em SIAM Journal on Scientific Computing}, 31(5):3744--3759, 2009.

\bibitem[Sie39]{Siegel:1939}
C.~L. Siegel.
\newblock {Einf{\"u}hrung in die Theorie der Modulfunktionen $n$-ten Grades}.
\newblock {\em Mathematische Annalen}, 116(1):617--657, 1939.

\bibitem[Swa08]{Swart:2008}
T.~C. Swart.
\newblock {\em {Initial Value Representations}}.
\newblock Dissertation, Freie Universit{\"a}t Berlin, 2008.

\bibitem[WRB04]{Worth:2004}
G.~A. Worth, M.~A. Robb, and I.~Burghardt.
\newblock {A novel algorithm for non-adiabatic direct dynamics using
  variational Gaussian wavepackets}.
\newblock {\em Faraday Discussions}, 127:307--323, 2004.

\bibitem[Zhe14]{Zheng:2014}
C.~Zheng.
\newblock {Optimal Error Estimates for First-Order Gaussian Beam Approximations
  to the Schr{\"o}dinger Equation}.
\newblock {\em SIAM Journal on Numerical Analysis}, 52(6):2905--2930, 2014.

\end{thebibliography}

